Causal Inference in Geosciences with Kernel Sensitivity Maps

Establishing causal relations between random variables from observational data is perhaps the most important challenge in today's Science. In remote sensing and geosciences this is of special relevance to better understand the Earth's system and the complex and elusive interactions between processes. In this paper we explore a framework to derive cause-effect relations from pairs of variables via regression and dependence estimation. We propose to focus on the sensitivity (curvature) of the dependence estimator to account for the asymmetry of the forward and inverse densities of approximation residuals. Results in a large collection of 28 geoscience causal inference problems demonstrate the good capabilities of the method.

==> data.tex <==
\begin{figure}[ht!]
\includegraphics[width=0.5\textwidth]{../matlab/ERMES_data_insitu_PROSAIL/figures/study_areas_ERMES_JGP.jpg}
\caption{Study areas and parcels where ground measurements were acquired.}
\label{fig:study_areas}
\end{figure}
Non-destructive real LAI data were acquired in the framework of the local ERMES field activities within rice fields in Spain, Italy and Greece (see Fig.~\ref{fig:study_areas}). The field campaigns were conducted during the 2014, 2015 and 2016 European rice seasons. During each season, the temporal frequency of the campaigns was approximately 10 day starting from the very beginning of rice emergence (early-June) up to the maximum rice green LAI development (mid-August). The same sampling scheme was used over each field following the guidelines and recommendations of the Validation of Land European Remote sensing Instruments (VALERI) protocol. LAI measurements were acquired using a dedicated smartphone app (PocketLAI) which uses both smartphone's accelerometer and camera to acquire images at 57.5º below the canopy and computes LAI through an internal segmentation algorithm~\cite{CamposTaberner2016a}. The center of the ESU was geo-located for later matching and associate the mean LAI estimate with the corresponding satellite spectra. In this study we used Landsat 8 surface reflectance data over each area corresponding to the dates of measurements' acquisition. On the other hand, the simulated data set (2000 pairs of Landsat 8 spectra and LAI) was obtained running the PROSAIL radiative transfer model in forward mode. PROSAIL simulates leaf reflectance for the optical spectrum from 400 to 2500 nm with a 1 nm spectral resolution and as a function of biochemistry and structure of the canopy, its leaves, the background soil reflectance and the sun-view geometry. The leaf and canopy variables as well as the soil brightness parameter, were randomly generated following a PROSAIL site-specific parameterization~\cite{CamposTaberner2016b} in order to constrain the behavior of the model to Mediterranean rice areas (see Fig.~\ref{tab:distributions}).
\begin{table}[!h]
\small
\begin{center}
\caption{Distribution of the canopy, leaf and soil parameters within the PROSAIL RTM.}
\label{tab:distributions}
\begin{adjustbox}{max width=0.48\textwidth}
\begin{tabular}{clccccc}
\toprule
\multicolumn{2}{c}{Parameter}                             & \multicolumn{1}{l}{Min} & \multicolumn{1}{l}{Max} & \multicolumn{1}{l}{Mode} & \multicolumn{1}{l}{Std} & Type         \\ \cmidrule(r){1-2} \cmidrule(r){3-7}
\multirow{4}{*}{Canopy} & LAI (m$^2$/m$^2$)                &0                         &10                         &3.5                          &4.5                         & Gaussian     \\
                        & ALA ($^\circ$)                          &30                         &80                         &60                          &20                         & Gaussian     \\
                        & Hotspot                          &0.1                         &0.5                         &0.2                          &0.2                         & Gaussian     \\
                        & vCover                          &0.5                        &1                         &1                          &0.2                        & Trunc. Gaussian     \\
\multirow{4}{*}{Leaf}   & N                                &1.2                         &2.2                         &1.5                          &0.3                         & Gaussian     \\
                        & C$_{ab}$ ($\mu$g$\cdot$cm$^{− 2}$) &20                         &90                         &45                          &30                         & Gaussian     \\
                        & C$_{dm}$ (g$\cdot$cm$^{− 2}$) &0.003                         &0.011                         &0.005                          &0.005                         & Gaussian     \\
                        & C$_{wREL}$                          &0.6                         &0.8                         &-                          &-                         & Uniform      \\
Soil                    & $\beta_{s}$                      &0.3   &1.2     &0.9     &0.25 & Gaussian \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

